The scenario-based generalization of radiation therapy margins

We give a scenario-based treatment plan optimization formulation that is equivalent to planning with geometric margins if the scenario doses are calculated using the static dose cloud approximation. If the scenario doses are instead calculated more accurately, then our formulation provides a novel robust planning method that overcomes many of the difficulties associated with previous scenario-based robust planning methods. In particular, our method protects only against uncertainties that can occur in practice, it gives a sharp dose fall-off outside high dose regions, and it avoids underdosage of the target in ``easy'' scenarios. The method shares the benefits of the previous scenario-based robust planning methods over geometric margins for applications where the static dose cloud approximation is inaccurate, such as irradiation with few fields and irradiation with ion beams. These properties are demonstrated on a suite of phantom cases planned for treatment with scanned proton beams subject to systematic setup uncertainty.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%
% LaTeX macros.tex
%%%%%%%%%%%%%%%%%%

\catcode`@=11

%  \def\proof{\penalty 25\noindent{\bf Proof.}\nobreak\hskip 1em\ignorespaces}
   \def\noproof{\hspace{1em}\blackslug}
  \def\mm#1{\hbox{$#1$}}                 % math mode
  \def\mtx#1#2{\renewcommand{\arraystretch}{1.2}%
      \left(\! \begin{array}{#1}#2\end{array}\! \right)}

%%% Miscellaneous items

\def\twonorm#1{\norm{#1}_2}
\def\onenorm#1{\norm{#1}_1}
\def\infnorm#1{\norm{#1}_{\infty}}
\def\disp{\displaystyle}
\def\m{\phantom-}
\def\EM#1{{\em#1\/}}
\def\ur{\mbox{\bf u}}
\def\Real{I\!\!R}
\def\Re{I\!\!R}
\def\FR{I\!\!F}
\def\Complex{I\mskip -11.3mu C}
\def\sp{\hspace{10pt}}
\def\subject{\operator@font subject\ to}
\def\minimize#1{{\displaystyle\minim_{#1}}} 
\def\minimizearg#1#2{{\displaystyle\minim_{#1 \in \Re^{#2}}}} 
\def\minimizetwoarg#1#2#3#4{{\displaystyle\minim_{#1 \in \Re^{#2},%
                                                  #3 \in \Re^{#4}}}}
\def\maximize#1{{\displaystyle\maxim_{#1}}} 
\def\eval#1#2{\left.#2\right|_{\alpha=#1}}

\def\tmat#1#2{(\, #1 \ \ #2 \,)}
\def\tmatt#1#2#3{(\, #1 \ \  #2 \ \  #3\,)}
\def\tmattt#1#2#3#4{(\, #1 \ \  #2 \ \  #3 \ \  #4\,)}

\def\mat#1#2{(\; #1 \quad #2 \;)}
\def\matt#1#2#3{(\; #1 \quad #2 \quad #3\;)}
\def\mattt#1#2#3#4{(\; #1 \quad #2 \quad #3 \quad #4\;)}
\def\blackslug{\hbox{\hskip 1pt \vrule width 4pt height 6pt depth 1.5pt
  \hskip 1pt}}
\def\boxit#1{\vbox{\hrule\hbox{\vrule\hskip 3pt
  \vbox{\vskip 3pt #1 \vskip 3pt}\hskip 3pt\vrule}\hrule}}
\def\cross{\scriptyscriptstyle\times}
\def\maxim{\mathop{\operator@font maximize}}
\def\minim{\mathop{\operator@font minimize}}
\def\cond{\mathop{\operator@font cond}}
\def\diag{\mathop{\operator@font diag}}
\def\dim{\mathop{\operator@font dim}}
\def\In{\mathop{\operator@font In}}
\def\dom{\mathop{\operator@font dom}}
\def\dist{\mathop{\operator@font dist}}
\def\boundary{\mathop{\operator@font bnd}}
\def\interior{\mathop{\operator@font int}}
\def\Null{\mathop{\operator@font null}}
\def\rank{\mathop{\operator@font rank}}
\def\op{\mathop{\operator@font op}}
\def\range{\mathop{\operator@font range}}
\let\Range\range
\def\epi{\mathop{\operator@font epi}}
\def\sign{\mathop{\operator@font sign}}
\def\sgn{\mathop{\operator@font sgn}}
\def\Span{\mathop{\operator@font span}}
\def\trace{\mathop{\operator@font trace}}
\def\drop{^{\null}}
\def\etal{{\em et al.\ }}  %%% e.g., Gill \etal (1986)
\def\float{fl}
\def\grad{\nabla}
\def\Hess{\nabla^2}
% \def\half  {{\textstyle{1\over 2}}}
% \def\third {{\textstyle{1\over 3}}}
% \def\fourth{{\textstyle{1\over 4}}}
% \def\sixth{{\textstyle{1\over 6}}}
\def\half  {{\textstyle{\frac12}}}
\def\third {{\textstyle{\frac13}}}
\def\fourth{{\textstyle{\frac14}}}
\def\sixth{{\textstyle{\frac16}}}
\def\inv{^{-1}}
\def\psinv{^{\dag}}
\def\invsq{^{-2}}
\def\limk{\lim_{k\to\infty}}
\def\mystrut{\vrule height10.5pt depth5.5pt width0pt}
\def\mod#1{|#1|}
\let\abs\mod
\def\modd#1{\biggl|#1\biggr|}
\def\Mod#1{\left|#1\right|}
\def\normm#1{\biggl\|#1\biggr\|}
\def\norm#1{\|#1\|}
\def\spose#1{\hbox to 0pt{#1\hss}}
\def\sub#1{^{\null}_{#1}}
\def\text #1{\hbox{\quad#1\quad}}
\def\textt#1{\hbox{\qquad#1\qquad}}
\def\T{^T\!}
\def\Tinv{^{-T}\!}
\def\ntext#1{\noalign{\vskip 2pt\hbox{#1}\vskip 2pt}}
\def\enddef{{$\null$}}
\def\xint{{x_{\rmfamily int}}}
\def\vhat{{\hat v}}

%%% Fixed-size glue, only for math mode

\def\pthinsp{\mskip  2   mu}    %           thin space
\def\pmedsp {\mskip  2.75mu}    %         medium space
\def\pthiksp{\mskip  3.5 mu}    %          thick space
\def\nthinsp{\mskip -2   mu}
\def\nmedsp {\mskip -2.75mu}
\def\nthiksp{\mskip -3.5 mu}

%%% Specially lowered subscripts (see \sub above)

\def\Asubk{A\sub{\nthinsp k}}
\def\Bsubk{B\sub{\nthinsp k}}
\def\Fsubk{F\sub{\nmedsp k}}
\def\Gsubk{G\sub{\nthinsp k}}
\def\Hsubk{H\sub{\nthinsp k}}
\def\HsubB{H\sub{\nthinsp \scriptscriptstyle{B}}}
\def\HsubS{H\sub{\nthinsp \scriptscriptstyle{S}}}
\def\HsubBS{H\sub{\nthinsp \scriptscriptstyle{BS}}}
\def\Hz{H\sub{\nthinsp \scriptscriptstyle{Z}}}
\def\Jsubk{J\sub{\nmedsp k}}
\def\Psubk{P\sub{\nthiksp k}}
\def\Qsubk{Q\sub{\nthinsp k}}
\def\Vsubk{V\sub{\nmedsp k}}
\def\Vsubone{V\sub{\nmedsp 1}}
\def\Vsubtwo{V\sub{\nmedsp 2}}
\def\Ysubk{Y\sub{\nmedsp k}}
\def\Wsubk{W\sub{\nthiksp k}}
\def\Zsubk{Z\sub{\nthinsp k}}
\def\Zsubi{Z\sub{\nthinsp i}}

%%% Subscripts

\def\subfr{_{\scriptscriptstyle{\it FR}}}
\def\subfx{_{\scriptscriptstyle{\it FX}}}
\def\fr{_{\scriptscriptstyle{\it FR}}}
\def\fx{_{\scriptscriptstyle{\it FX}}}
\def\submax{_{\max}}
\def\submin{_{\min}}
\def\subminus{_{\scriptscriptstyle -}}
\def\subplus {_{\scriptscriptstyle +}}

\def\A{_{\scriptscriptstyle A}}
\def\B{_{\scriptscriptstyle B}}
\def\BS{_{\scriptscriptstyle BS}}
\def\C{_{\scriptscriptstyle C}}
\def\D{_{\scriptscriptstyle D}}
\def\E{_{\scriptscriptstyle E}}
\def\F{_{\scriptscriptstyle F}}
\def\G{_{\scriptscriptstyle G}}
\def\H{_{\scriptscriptstyle H}}
\def\I{_{\scriptscriptstyle I}}
\def\w{_w}
\def\k{_k}
\def\kp#1{_{k+#1}}
\def\km#1{_{k-#1}}
\def\j{_j}
\def\jp#1{_{j+#1}}
\def\jm#1{_{j-#1}}
\def\K{_{\scriptscriptstyle K}}
\def\L{_{\scriptscriptstyle L}}
\def\M{_{\scriptscriptstyle M}}
\def\N{_{\scriptscriptstyle N}}
\def\suba{\A}
\def\subb{\B}
\def\subbbar{_{\scriptscriptstyle \bar B}}
\def\subc{\C}
\def\subm{\M}
\def\subf{\F}
\def\subn{\N}
\def\subh{\H}
\def\subk{\K}
\def\subp{_{\scriptscriptstyle P}}
\def\subt{_{\scriptscriptstyle T}}
\def\subr{\R}
\def\subz{\Z}
\def\J{_{\scriptscriptstyle J}}
\def\O{_{\scriptscriptstyle O}}
\def\Q{_{\scriptscriptstyle Q}}
\def\P{_{\scriptscriptstyle P}}
\def\R{_{\scriptscriptstyle R}}
\def\S{_{\scriptscriptstyle S}}
\def\U{_{\scriptscriptstyle U}}
\def\V{_{\scriptscriptstyle V}}
\def\W{_{\scriptscriptstyle W}}
\def\Y{_{\scriptscriptstyle Y}}
\def\Z{_{\scriptscriptstyle Z}}

%%% Superscript stars

\def\superstar{^{\raise 0.5pt\hbox{$\nthinsp *$}}}
\def\SUPERSTAR{^{\raise 0.5pt\hbox{$*$}}}
\def\shrink{\mskip -7mu}  %%% Less space after \xstar if followed by , or .

\def\alphastar{\alpha\superstar}
\def\lamstar  {\lambda\superstar}
\def\lamstarT {\lambda^{\raise 0.5pt\hbox{$\nthinsp *$}T}}
\def\lambdastar{\lamstar}
\def\nustar{\nu\superstar}
\def\mustar{\mu\superstar}
\def\pistar{\pi\superstar}

\def\cstar{c\superstar}
\def\dstar{d\SUPERSTAR}
\def\fstar{f\SUPERSTAR}
\def\gstar{g\superstar}
\def\hstar{h\superstar}
\def\mstar{m\superstar}
\def\pstar{p\superstar}
\def\sstar{s\superstar}
\def\ustar{u\superstar}
\def\vstar{v\superstar}
\def\wstar{w\superstar}
\def\xstar{x\superstar}
\def\ystar{y\superstar}
\def\zstar{z\superstar}

\def\Astar{A\SUPERSTAR}
\def\Bstar{B\SUPERSTAR}
\def\Cstar{C\SUPERSTAR}
\def\Fstar{F\SUPERSTAR}
\def\Gstar{G\SUPERSTAR}
\def\Hstar{H\SUPERSTAR}
\def\Jstar{J\SUPERSTAR}
\def\Kstar{K\SUPERSTAR}
\def\Mstar{M\SUPERSTAR}
\def\Ustar{U\SUPERSTAR}
\def\Vstar{V\SUPERSTAR}
\def\Wstar{W\SUPERSTAR}
\def\Xstar{X\SUPERSTAR}
\def\Zstar{Z\SUPERSTAR}

%%% bars, hats, tildes  (\skew4 is the default)

\def\alphabar{\bar \alpha}
\def\alphahat{\skew3\hat \alpha}
\def\alphatilde{\skew3\tilde \alpha}
\def\betabar{\skew{2.8}\bar\beta}
\def\betahat{\skew{2.8}\hat\beta}
\def\betatilde{\skew{2.8}\tilde\beta}
\def\delbar{\bar\delta}
\def\deltilde{\skew5\tilde \delta}
\def\deltabar{\delbar}
\def\deltatilde{\deltilde}
\def\lambar{\bar\lambda}
\def\etabar{\bar\eta}
\def\gammabar{\bar\gamma}
\def\lamhat{\skew{2.8}\hat \lambda}
\def\lambdabar{\lambar}
\def\lambdahat{\lamhat}
\def\mubar{\skew3\bar \mu}
\def\muhat{\skew3\hat \mu}
\def\mutilde{\skew3\tilde\mu}
\def\nubar{\skew3\bar\nu}
\def\nuhat{\skew3\hat\nu}
\def\nutilde{\skew3\tilde\nu}
\def\omegabar{\bar\omega}
\def\pibar{\bar\pi}
\def\pihat{\skew1\widehat \pi}
\def\sigmabar{\bar\sigma}
\def\rhobar{\bar\rho}
\def\rhohat{\widehat\rho}
\def\taubar{\bar\tau}
\def\tautilde{\tilde\tau}
\def\tauhat{\hat\tau}
\def\thetabar{\bar\theta}
\def\xibar{\skew4\bar\xi}

\def\superplus{{^{\scriptscriptstyle +}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Math italic and calligraphic fonts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Deltait{{\mit \Delta}}
\def\Gammait{{\mit \Gamma}}
\def\Lambdait{{\mit \Lambda}}
\def\Sigmait{{\mit \Sigma}}
\def\Lambarit{\skew5\bar{\mit \Lambda}}
\def\Omegait{{\mit \Omega}}
\def\Omegaitbar{\skew5\bar{\mit \Omega}}
\def\Thetait{{\mit \Theta}}
\def\Piitbar{\skew5\bar{\mit \Pi}}
\def\Piit{{\mit \Pi}}
\def\Phiit{{\mit \Phi}}
\def\Xiit{{\mit \Xi}}
\def\Ascr{{\cal A}}
\def\Bscr{{\cal B}}
\def\Fscr{{\cal F}}
\def\Dscr{{\cal D}}
\def\Iscr{{\cal I}}
\def\Jscr{{\cal J}}
\def\Lscr{{\cal L}}
\def\Mscr{{\cal M}}
\def\lscr{\ell}
\def\lscrbar{\ellbar}
\def\Oscr{{\cal O}}
\def\Pscr{{\cal P}}
\def\Qscr{{\cal Q}}
\def\Sscr{{\cal S}}
\def\Uscr{{\cal U}}
\def\Vscr{{\cal V}}
\def\Wscr{{\cal W}}
\def\Mscr{{\cal M}}
\def\Nscr{{\cal N}}
\def\Rscr{{\cal R}}

\def\abar{\skew3\bar a}
\def\ahat{\skew2\widehat a}
\def\atilde{\skew2\widetilde a}
\def\Abar{\skew7\bar A}
\def\Ahat{\widehat A}
\def\Atilde{\widetilde A}
\def\bbar{\skew3\bar b}
\def\bhat{\skew2\widehat b}
\def\btilde{\skew2\widetilde b}
\def\Bbar{\bar B}
\def\Bhat{\widehat B}
\def\cbar{\skew5\bar c}
\def\chat{\skew3\widehat c}
\def\ctilde{\widetilde c}
\def\Cbar{\bar C}
\def\Chat{\widehat C}
\def\Ctilde{\widetilde C}
\def\dbar{\bar d}
\def\dhat{\widehat d}
\def\dtilde{\widetilde d}
\def\Dbar{\bar D}
\def\Dhat{\widehat D}
\def\Dtilde{\widetilde D}
\def\ehat{\skew3\widehat e}
\def\ebar{\bar e}
\def\Ebar{\bar E}
\def\Ehat{\widehat E}
\def\fbar{\bar f}
\def\fhat{\widehat f}
\def\ftilde{\widetilde f}
\def\Fbar{\bar F}
\def\Fhat{\widehat F}
\def\gbar{\skew{4.3}\bar g}
\def\ghat{\skew{4.3}\widehat g}
\def\gtilde{\skew{4.5}\widetilde g}
\def\Gbar{\bar G}
\def\Ghat{\widehat G}
\def\hbar{\skew{4.2}\bar h}
\def\hhat{\skew2\widehat h}
\def\htilde{\skew3\widetilde h}
\def\Hbar{\skew5\bar H}
\def\Hhat{\widehat H}
\def\Htilde{\widetilde H}
\def\Ibar{\skew5\bar I}
\def\Itilde{\widetilde I}
\def\Jbar{\skew6\bar J}
\def\Jhat{\widehat J}
\def\Jtilde{\widetilde J}
\def\kbar{\skew{4.4}\bar k}
\def\Khat{\widehat K}
\def\Kbar{\skew{4.4}\bar K}
\def\Ktilde{\widetilde K}
\def\ellbar{\bar \ell}
\def\lhat{\skew2\widehat l}
\def\lbar{\skew2\bar l}
\def\Lbar{\skew{4.3}\bar L}
\def\Lhat{\widehat L}
\def\Ltilde{\widetilde L}
\def\mbar{\skew2\bar m}
\def\mhat{\widehat m}
\def\Mbar{\skew{4.4}\bar M}
\def\Mhat{\widehat M}
\def\Mtilde{\widetilde M}
\def\Nbar{\skew{4.4}\bar N}
\def\Ntilde{\widetilde N}
\def\nbar{\skew2\bar n}
\def\pbar{\skew2\bar p}
%\def\phat{\skew2\widehat p}
\def\phat{\skew2\widehat p}
\def\ptilde{\skew2\widetilde p}
\def\Pbar{\skew5\bar P}
\def\Phat{\widehat P}
\def\Ptilde{\skew5\widetilde P}
\def\qbar{\bar q}
\def\qhat{\skew2\widehat q}
\def\qtilde{\widetilde q}
\def\Qbar{\bar Q}
\def\Qhat{\widehat Q}
\def\Qtilde{\widetilde Q}
\def\rbar{\skew3\bar r}
\def\rhat{\skew3\widehat r}
\def\rtilde{\skew3\widetilde r}
\def\Rbar{\skew5\bar R}
\def\Rhat{\widehat R}
\def\Rtilde{\widetilde R}
\def\sbar{\bar s}
\def\shat{\widehat s}
\def\Stilde{\widetilde S}
\def\stilde{\widetilde s}
\def\Shat{\widehat S}
\def\Sbar{\skew2\bar S}
\def\tbar{\bar t}
\def\ttilde{\widetilde t}
\def\that{\widehat t}
\def\Tbar{\bar T}
\def\That{\widehat T}
\def\Ttilde{\widetilde T}
\def\ubar{\skew3\bar u}
\def\uhat{\skew3\widehat u}
\def\utilde{\skew3\widetilde u}
\def\Ubar{\skew2\bar U}
\def\Uhat{\widehat U}
\def\Utilde{\widetilde U}
\def\vbar{\skew3\bar v}
\def\vhat{\skew3\widehat v}
\def\vtilde{\skew3\widetilde v}
\def\Vbar{\skew2\bar V}
\def\Vhat{\widehat V}
\def\Vtilde{\widetilde V}
\def\wbar{\skew3\bar w}
\def\what{\skew3\widehat w}
\def\wtilde{\skew3\widetilde w}
\def\Wbar{\skew3\bar W}
\def\What{\widehat W}
\def\Wtilde{\widetilde W}
\def\xbar{\skew{2.8}\bar x}
\def\xhat{\skew{2.8}\widehat x}
\def\xtilde{\skew3\widetilde x}
\def\Xhat{\widehat X}
\def\ybar{\skew3\bar y}
\def\yhat{\skew3\widehat y}
\def\ytilde{\skew3\widetilde y}
\def\Ytilde{\widetilde Y}
\def\Ybar{\skew2\bar Y}
\def\Yhat{\widehat Y}
\def\zbar{\skew{2.8}\bar z}
\def\zhat{\skew{2.8}\widehat z}
\def\ztilde{\skew{2.8}\widetilde z}
\def\Zbar{\skew5\bar Z}
\def\Zhat{\widehat Z}
\def\Ztilde{\widetilde Z}
\def\MINOS{{\small MINOS}}
\def\NPSOL{{\small NPSOL}}
\def\QPSOL{{\small QPSOL}}
\def\LUSOL{{\small LUSOL}}
\def\LSSOL{{\small LSSOL}}
\def\implies{\Rightarrow}

\def\argmin{\mathop{\operator@font argmin}}
\def\argmax{\mathop{\operator@font argmax}}
\def\conv{\mathop{\operator@font conv}}

\def\defined{\buildrel{\scriptscriptstyle\triangle}\over=}

\catcode`@=12

